The Involutive Quantaloid of Completely Distributive Lattices

Let L be a complete lattice and let Q(L) be the unital quantale of join-continuous endo-functions of L. We prove the following result: Q(L) is an involutive (that is, non-commutative cyclic $\star$-autonomous) quantale if and only if L is a completely distributive lattice. If this is the case, then the dual tensor operation corresponds, via Raney's transforms, to composition in the (dual) quantale of meet-continuous endo-functions of L. Let sLatt be the category of sup-lattices and join-continuous functions and let cdLatt be the full subcategory of sLatt whose objects are the completely distributive lattices. We argue that (i) cdLatt is itself an involutive quantaloid, and therefore it is the largest full-subcategory of sLatt with this property; (ii) cdLatt is closed under the monoidal operations of sLatt and, consequently, if Q(L) is involutive, then Q(L) is completely distributive as well.

==> cdlatt.tex <==
\section{\Cdlatt{s}}
In this appendix we sketch a proof of Theorem~\ref{thm:raney}. Since
the proof is essentially the same as in Raney's paper \cite{Raney60},
we do not include it in the main text.

Let us consider the condition
\begin{align}
  \label{eq:meetofO}
  \bigwedge_{\COND{t}{y}} o_{L}(t)
  &  = y\,.
\end{align}
    
We firstly (in the following lemma) observe that
condition~\eqref{eq:meetofO} is autodual. Let us remark, however, that this shall also be
a consequence of Theorem~\ref{thm:characterization}, characterising
the lattices satisfying the dual of equation~\eqref{eq:meetofO} as the
completely distributive lattices (it is well-known that in a classical
context, the condition defining a \cdlatt is autodual).
\begin{lemma}
  Condition~\eqref{eq:meetofO} is autodual.
\end{lemma}
\begin{Proof}
  We need to show that condition~\eqref{eq:meetofO} implies the
  following one:
  \begin{align}
    \label{eq:joinofO}
    x & = \bigvee_{x \not\leq t} \omega_{L}(t)\,. 
  \end{align}
  That is, we need to show that if $y$ is such that
  $\omega_{L}(t) \leq y$ whenever $x \not \leq t$, then $x \leq
  y$. Now, to achieve this goal, we fix such a $y$, take $u$ such that
  $u \not\leq y$ and, on view of \eqref{eq:meetofO}, we show then that
  $x \leq o_{L}(u)$.  Indeed, if $x \not\leq o_{L}(u)$, then
  $\omega_{L}(o_{L}(u)) \leq y$, and considering that
  $u \leq \omega_{L}(o_{L}(u))$, then we get $u \leq y$, a \contr.
\end{Proof}

\begin{theorem}
  \label{thm:characterization}
  A complete lattice satisfies condition~\eqref{eq:joinofO} if and
  only if it is \cd.
\end{theorem}
\begin{Proof}
  We firstly argue that if a lattice $L$
  satisfies~\eqref{eq:joinofO}, then it is \cd.
  Let $\pi : J \rto I$ be a family, and write $J_{i} =
  \pi^{-1}(i)$. We argue that
  \begin{align*}
    \bigwedge_{i \in I} \bigvee_{j \in J_{i}} x_{i,j} & \leq
    \bigvee_{\pi \circ f = id_{I}} \bigwedge_{i \in I} x_{i,f(i)}\,.
  \end{align*}
  Let $y = \bigwedge_{i \in I} \bigvee_{j \in J_{i}} x_{i,j}$, we
  shall show that if $\COND{y}{t}$ and $\omega_{L}(t) \leq y$, then
  there exists a choice function $f : I \rto J$ (thus such that
  $\pi \circ f = id_{I}$) with
  $\omega_{L}(t) \leq \bigwedge_{i \in I} x_{i,f(i)}$.

  For each $i \in I$, we have
  $\omega_{L}(t) \leq \bigvee_{j \in J_{i}} x_{i,j}\not\leq t$, and
  therfore there exists $f(i)$ such that $x_{i,f(i)} \not\leq t$.
  Notice that the condition $x_{i,f(i)} \not\leq t$ implues
  $\omega_{L}(t) \leq x_{i,f(i)}$.  We have therefore
  $\omega_{L}(t) \leq x_{i,f(i)}$, for each $i \in I$, and therefore
  $\omega_{L}(t) \leq \bigwedge_{i \in I} x_{i,f(i)}$.

  We argue now that if $L$ is completely distributive,
  then~\eqref{eq:joinofO} holds.  The inclusion
  $\bigvee_{x \not\leq t} \omega_{L}(t) \leq x$ always holds and
  therefore we only argue for the opposite inclusion.  By complete
  distributivity, we have
  \begin{align*}
    \bigvee_{x \not\leq t} \omega_{L}(t) & = \bigvee_{x \not\leq t}
    \bigwedge_{u \not\leq t} u = \bigwedge_{f} \bigvee_{x \not\leq t}
    f(t)\,,
  \end{align*}
  where the last meet is taken over all functions
  $f : \set{ t \mid x \not\leq t} \rto L$ such that $f(t) \not\leq t$.
  Therefore, to argue that
  $x \leq \bigvee_{x \not\leq t} \omega_{L}(t)$, it shall be enough to
  consider an arbitrary such function and show that
  $x \leq \bigvee_{x \not\leq t} f(t)$.  Let
  $t_{f} = \bigvee_{x \not\leq t} f(t)$ and suppose, by contradiction,
  that $x \not \leq t_{f}$. It follows then that $f$ is defined on
  $t_{f}$ and consequently
  $f(t_{f}) \leq \bigvee_{x \not\leq t} f(t) = t_{f}$.  However, this
  contradicts the requirement that $f(t_{f}) \not\leq t_{f}$.
\end{Proof}





==> macros.tex <==
\RequirePackage{xspace}
\RequirePackage{textlogic}
\RequirePackage{color}
\input{theorems}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{#1}
\newcommand{\BOF}{\red{BOOF ???}}

\newcommand{\intfun}{\,\cdot\,}
\newcommand{\fun}[1]{(\,\cdot\,)^{#1}}
\newcommand{\meetof}[1]{{#1}{}^{\land}}
\newcommand{\joinof}[1]{{#1}{}^{\vee}}
\newcommand{\funJoinOf}{\fun{\vee}}
\newcommand{\funMeetOf}{\fun{\land}}
\newcommand{\MEETOF}{\funMeetOf}
\newcommand{\JOINOF}{\funJoinOf}
\newcommand{\DUAL}{\fun{\partial}}
\newcommand{\dual}[1]{#1^{\partial}}
\newcommand{\STAR}{\fun{\star}}
\newcommand{\Star}[1]{#1{}^{\star}}

\newif\ifAbstract
\Abstractfalse

\ifAbstract
\newcommand{\mc}{meet-preserving\xspace}
\newcommand{\jc}{sup-preserving\xspace}
\newcommand{\jmc}{join/meet-preserving\xspace}
\else
\newcommand{\mc}{meet-continuous\xspace}
\newcommand{\jc}{join-continuous\xspace}
\newcommand{\jmc}{join/meet-continuous\xspace}
\fi
\newcommand{\contr}{contradiction\xspace}
\newcommand{\cjp}{completely join-prime\xspace}
\newcommand{\cjirr}{completely join-irreducible\xspace}
\newcommand{\cmirr}{completely meet-irreducible\xspace}
\newcommand{\cmp}{completely meet-prime\xspace}
\newcommand{\rto}[1][\;]{\xrightarrow{\;\;#1\;\;}}
\newcommand{\ddownarrow}{\,\downarrow\!\!\downarrow}
\newcommand{\eqdef}{:=}
\newcommand{\ra}[1]{\rho(#1)}
\newcommand{\la}[1]{\ell(#1)}
\newcommand{\radj}{right adjoint\xspace}
\newcommand{\ladj}{left adjoint\xspace}

\newcommand{\set}[1]{\{ \,#1\, \}}

\newcommand{\Q}{{\mathcal{Q}}} 
\newcommand{\D}{{\mathcal{D}}} 
\newcommand{\QD}{\Q(D)} 
\newcommand{\DP}{\D(P)} 
\newcommand{\QDP}{\Q(\D(P))} 
\newcommand{\QL}{\Q(L)} 
\newcommand{\QC}{\Q(C)} 
\newcommand{\C}{{\mathcal{C}}} 
\newcommand{\R}{{\mathbb{R}}} 

\ifAbstract
\newcommand{\SLatt}{\text{Sup-Latt}\xspace} 
\newcommand{\CDLatt}{\text{Cd-\SLatt}\xspace} 
\else
\newcommand{\SLatt}{\ensuremath{\mathsf{Latt}_{\bigvee}}\xspace} 
\newcommand{\CDLatt}{\ensuremath{\SLatt^{\mathtt{cd}}}\xspace} 
\fi
\newcommand{\MLatt}{\ensuremath{\mathsf{Latt}_{\bigwedge}}\xspace} 

\newcommand{\iq}{involutive quantaloid\xspace}
\newcommand{\Iq}{Involutive quantaloid\xspace}
\newcommand{\iqe}{involutive quantale\xspace}
\newcommand{\qe}{quantale\xspace}
\newcommand{\rl}{residuated lattice\xspace}
\newcommand{\irl}{involutive \rl}
\newcommand{\upon}{/}
\newcommand{\below}{\backslash}

\tikzset{
    labl/.style={rotate=90}
}

\newcommand{\commTriangle}[6]{
  \begin{tikzcd}[ampersand replacement=\&]
    #1 \ar[rd, "#4"] \ar[rr, "#6"]\& {} \& #3 \\
    \& #2 \ar[ru, "#5"]\ar[phantom, u, "\leq" labl] \&
  \end{tikzcd}
}

\newcommand{\cjh}{complete join-homomorphism\xspace} 
\newcommand{\cond}[2]{#1 < #2} 
\newcommand{\Cond}[2]{#2 \not\leq #1} 
\newcommand{\COND}[2]{#1 \not\leq #2} 
\newcommand{\fantastic}{fantastic\xspace} 
\newcommand{\jfantastic}{join-\fantastic} 
\newcommand{\mfantastic}{meet-\fantastic} 
\renewcommand{\int}{\mathtt{int}}
\newcommand{\cl}{\mathtt{cl}}
\newcommand{\clatt}{complete lattice\xspace}
\newcommand{\cc}{complete chain\xspace}
\newcommand{\cdlatt}{\cd lattice\xspace}
\newcommand{\Cdlatt}{\Cd lattice\xspace}
\newcommand{\twocomp}{$2$-compatible\xspace}
\newcommand{\cd}{completely distributive\xspace}
\newcommand{\Cd}{Completely distributive\xspace}
\newcommand{\bigWedge}{\bigwedge\!\!\!\!\!\!\!\bigwedge}
\newcommand{\sg}{semigroup\xspace}

\renewcommand{\tiff}{\text{iff}\xspace}


\newenvironment{thm}{\vskip 6pt\par\noindent{\bf Theorem.~}\em}{\par\vskip 6pt}
\newenvironment{prop}[1]{\vskip 6pt\par\noindent{\bf Proposition~#1.~}\em}{\par\vskip 6pt} 
\newenvironment{cor}{\vskip 6pt\par\noindent{\bf Corollary.~}\em}{\par\vskip 6pt}

\newcommand{\propno}{2.6.18\xspace}





==> theorems.tex <==
\ifams
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{claim}{Claim}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem*{problem}{Problem}
\theoremstyle{remark}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\fi

\ifams
\newenvironment{Proof}{\begin{proof}}{\end{proof}}
\newenvironment{myproof}[1][]{
  \ifx&#1&
  \begin{proof}
    \else
    \begin{proof}[Proof of #1]
      \fi}{\end{proof}}
\else
\newcommand{\qedhere}{\qed}
\newenvironment{Proof}{\begin{proof}}{\qed\end{proof}}
\newenvironment{ProofNoQED}{\begin{proof}}{\end{proof}}
\newenvironment{myproof}[1][]{
  \ifx&#1&
  \begin{proof}
  \else
  \begin{proof}[#1]
  \fi
  }{\hfill\qed\end{proof}}
\fi



